Filter Distillation for Network Compression

In this paper we introduce Principal Filter Analysis (PFA), an easy to use and effective method for neural network compression. PFA exploits the correlation between filter responses within network layers to recommend a smaller network that maintain as much as possible the accuracy of the full model. We propose two algorithms: the first allows users to target compression to specific network property, such as number of trainable variable (footprint), and produces a compressed model that satisfies the requested property while preserving the maximum amount of spectral energy in the responses of each layer, while the second is a parameter-free heuristic that selects the compression used at each layer by trying to mimic an ideal set of uncorrelated responses. Since PFA compresses networks based on the correlation of their responses we show in our experiments that it gains the additional flexibility of adapting each architecture to a specific domain while compressing. PFA is evaluated against several architectures and datasets, and shows considerable compression rates without compromising accuracy, e.g., for VGG-16 on CIFAR-10, CIFAR-100 and ImageNet, PFA achieves a compression rate of 8x, 3x, and 1.4x with an accuracy gain of 0.4%, 1.4% points, and 2.4% respectively. Our tests show that PFA is competitive with state-of-the-art approaches while removing adoption barriers thanks to its practical implementation, intuitive philosophy and ease of use.

==> state_of_art_full.tex <==
\section{Related work}
\label{soa}





The field of network compression encompasses a wide range of techniques and relevant work can be grouped into four main categories: quantization, knowledge distillation, tensor factorization and network pruning. For an extensive review on network compression see~\citet{Cheng:SPM:2017}. 

Quantization algorithms compress networks by reducing the number of bits used to represent each weight~\citep{Jiaxiang:CVPR:2016,Han:ICLR:2016,Rastegari:ECCV:2016}. Quantization can be applied by learning binary weights during training or as a post-process. However, these algorithms often ignore the effect of binarization on the accuracy loss, resulting in a degradation of accuracy. A recent technique~\citep(He:ECCV2018) introduces a re-normalization step in order to 
restore the statistics in batch normalization and reduce accuracy degradation. \citet{Wu:ICML:2018} proposes to compress the network by sharing weights that are pre-computed by k-mean clustering.

Knowledge distillation~\citep{Hinton:NIPS:2014} and model compression~\citep{Bucilua:SIGKDD:2006} aim to create a simpler model that mimics the output of a more complex one. Variations on this concept include~\citep{Ba:NIPS:2014,Romero:ICRL:2015,Chen:ICLR:2016}. However, the design of the simpler model (i.e., shallower networks) is still an empirical process.

Tensor factorization algorithms exploit the redundancy present in convolution layers by replacing the original tensors with a sequence of smaller or sparser counterparts~\citep{Denton:NIPS:2014,Lebedev:ICLR:2015,Jaderberg:BMVC:2014,Tai:ICLR:2016,Masana:ICCV:2017,Yu:CVPR:2017,Peng:ECCV2018}. These techniques share with PFA the intuition about exploiting redundancy within a tensor. While PFA uses the concept of correlation within the responses, these techniques aim to find a new set of filters that minimizes the reconstruction error of the feature maps or the response output. Another difference with PFA is that these techniques, with the exception of \citet{Tai:ICLR:2016} and~\citet{Aghasi:NIPS:2017}, need to operate on one layer at the time. In contrast PFA can compress all layers simultaneously.

Network pruning is a family of techniques that compress networks by iteratively removing connections based on the saliency of their weights.  Early work, like Optimal Brain Damage~\citep{Lecun:NIPS:1990} and Optimal Brain Surgeon~\citep{Hassibi:NIPS:1993}, targeted fully connected networks by examining the Hessian of the loss function. Recent work can be divided into two sub-families: sparse pruning, where individual neurons are removed, and structured pruning, where entire filters are removed. 

Within sparse pruning, some works remove connections that play an insignificant role and retrain the network~\citep{Han:NIPS:2015}. \citet{Srinivas:BMVC:2015} propose a data-free parameter pruning for networks with fully connected layers where redundant neurons are iteratively removed. \citet{Tung:CVPR:2018} combines quantization and pruning in a joint learning framework.
Another trend, is to train compact networks by using sparsity inducing regularizers~\citep{Wen:NIPS:2016}. Other works formulate pruning as an optimization problem \citep{Aghasi:NIPS:2017, Carreira:CVPR:2018, Zahng:ECCV:2018}.

Structured pruning is a more intuitive compression technique and works on standard architectures and hardware. Some approaches focus explicitly on filter pruning, such as~\citet{Li:ICLR:2017}, where those filters with an $ \ell_1 $-norm smaller than a given threshold are removed. The threshold, however, remains a difficult parameter to tune since different layers require different thresholds. Other techniques choose which filter to remove by minimizing the reconstruction error of the filters' responses~\citep{He:ICCV:2017,Luo:ICCV:2017,Yu:CVPR:2018}. In~\citet{Liu:ICCV:2017}, sparsity is first induced during a new training phase and used to identify filters with weights close to zero. They propose an iterative strategy, with repeated training and pruning, to achieve acceptable accuracy. The main disadvantage of this approach is that it requires an additional training phase to induce sparsity. The effect on the final footprint and accuracy is hard to predict in advance. In recent work~\citep{Molchanov:ICLR:17}, filters that contribute least to the loss change are pruned by approximating the effect of a filter on the loss using Taylor expansion, and incorporating the approximation in a combinatorial optimization.

Within the structured pruning family, there are approaches based on the singular value decomposition (SVD) of the filter weights~\citep{Xue:ICASSP:2013, Nakkiran:IS:2015, Prabhavalkar:ICASSP:2016}. These techniques compute the SVD of the weights and replace the filters with a new set obtained by projection onto a lower dimensional subspace. Differences among these techniques are in the way the rank is estimated and how the projection is performed.

